Dependency-Based Neural Representations for Classifying Lines of Programs

We investigate the problem of classifying a line of program as containing a vulnerability or not using machine learning. Such a line-level classification task calls for a program representation which goes beyond reasoning from the tokens present in the line. We seek a distributed representation in a latent feature space which can capture the control and data dependencies of tokens appearing on a line of program, while also ensuring lines of similar meaning have similar features. We present a neural architecture, Vulcan, that successfully demonstrates both these requirements. It extracts contextual information about tokens in a line and inputs them as Abstract Syntax Tree (AST) paths to a bi-directional LSTM with an attention mechanism. It concurrently represents the meanings of tokens in a line by recursively embedding the lines where they are most recently defined. In our experiments, Vulcan compares favorably with a state-of-the-art classifier, which requires significant preprocessing of programs, suggesting the utility of using deep learning to model program dependence information.

==> discussion.tex <==
\section{Discussion}
The Natural Language Processing (NLP) and the PL analysis communities have the same task at hand - of reasoning about intent, given some text in a language.
While the specifics of the tasks differ, ..... 

The idea of incorporating program dependence information from ASTs, which we investigate in this work, is in the direction of recent efforts in NLP \cite{structure1, structure2, structure3, islstmgood}.
These works show that structural and hierarchical information from parse trees helps in training robust language models.
Moreover, since gathering meaning is a complex task and these representations capture a narrow aspect of it, we expect interest in an ensemble of models trained on different representations, perhaps even focusing on run-time behavior, will grow.

Maybe add future work where we say we'll also train just this representation in an unsupersived and then use it for downstream task. And specifically, do domain-general unsupervised and test on domain-specific supervision.





==> figures.tex <==
%<*overview>
\begin{figure*}[th]
        \resizebox{0.9\textwidth}{!}{
            \includegraphics[width=0.8\textwidth ]{img/overview.png}
%            \includegraphics[width=0.8\textwidth ]{img/um-staged-arch-fig-v1.pdf}
        }
        \caption{\textbf{Overview of \vulcan.} It uses the example of Figure \ref{flow1}. The inputs are the \thisline, i.e. \lfour, and the AST of the program. A representation for \lfour is computed, which is used by a classifier to predict whether that line has a vulnerability. In Stage~1, we backtrack to the line where a variable used on the current line was most recently defined. In Figure~\ref{flow1}, variables \texttt{y} and \texttt{r} were updated at \ltwo and \lthree. The path from the AST, expressing context in terms of control and data dependencies between \thisline and the most recent definition line, is then extracted. Each path, a sequence of length $s$,  is then passed, one at a time, to a bidirectional LSTM with dot-product attention to obtain its continuous-valued representation of dimension \texttt{q}. These intermediate \context representations are notated as $R{_C}(\cdot)$. In Stage~2 \context representations $R{_C}(\cdot)$ of all tokens are concatenated and passed through a feed forward network \texttt{FFN\_A} to obtain an intermediate representation (denoted in blue). In Stage~3,  the intermediate representation is concatenated with the \define representations (notated as $R_D(\cdot)$) of all the variables, and representations of operators. This concatenated vector is then transformed to a representation of dimension \texttt{t} using a feed forward network \texttt{FFN\_B}, which is the final representation for line \lfour, $R($\lfour$)$. See Algorithm \ref{algo} for details. This is then passed to a classifier \texttt{FFN\_C} to produce a binary value indicating presence of vulnerability}
        \label{overview}
\end{figure*}
%</overview>


%<*example>
\begin{figure}[hbt]
    \resizebox{\linewidth}{!}{
        \includegraphics[width=\linewidth]{img/example1.png}
    }
    \caption{An example code snippet. We show how different tokens and their dependencies can be represented. Paths comprising the nodes of a program AST represent both control and data information. Here, paths $\mathcal{P}_r, \mathcal{P}_y$ connect the usages of variables \texttt{r} and \texttt{y} on line \lfour to their respective updates on lines \ltwo and \lthree.}
    \label{flow1}
\end{figure}
%</example>

%<*errbarsz>
	\begin{minipage}
	\begin{minipage}[b]{0.49\textwidth}
		\begin{tabular}{lrrrrrr}
			\toprule
			Model &  F1 &  P & R & FPR & FNR & TPR \\
			\vulcan (This work) & 60 & 59 & 60 & 2 & 40 & 60\\ 
			\vuldl & 52 & 54 & 51 & 2 & 49 & 51\\ 
			\midrule
			\nb & 0 & 0 & 0 & 0 & 0 & 0\\ 
			\bowtok & 28 & 58 & 18 & 0 & 82 & 18\\ 
			\bowpath & 30 & 61 & 20 & 0 & 80 & 20\\ 
			\vullr & 52 & 54 & 51 & 2 & 49 & 51\\
			\vulcanab & 52 & 45 & 60 & 3 & 40 & 60\\ 
			\vulcanpl & 53 & 53 & 53 & 2 & 47 & 53\\ 
			\vulcanattn & 52 & 54 & 51 & 2 & 49 & 51\\ 
			\bottomrule
		\end{tabular}
		\caption{Vulnerability classification of different models evaluated in our work. 
			All values are percentages rounded to the nearest integer. 
			This is a binary classification task of classifying whether a line has a vulnerability or not. 
			The results are an average of 5 independent runs each.
			P, R stand for Precision and Recall respectively.}
		\label{table1}
	\end{minipage}
	\hfill
	\begin{minipage}[b]{0.49\textwidth}
	\resizebox{\linewidth}{!}{
		\includegraphics[width=\linewidth]{img/errbars.jpg}
	}
	\caption{An example code snippet. We motivate how different tokens and their dependencies can be represented. Paths comprising the nodes of a program AST represent both control and data information. Here, paths $\mathcal{P}_r, \mathcal{P}_y$ connect the usages of variables \texttt{r} and \texttt{y} on line \lfour to their respective updates on lines \ltwo and \lthree.}
	\label{errbars1}
	\end{minipage}
\end{minipage}
%</errbarsz>

%<*tabl>
\begin{table}[hbt]
\begin{tabular}{l|rrrrr}
		\toprule
		\textbf{Model} &  \textbf{F1} &  \textbf{P} & \textbf{R} & \textbf{FPR} & \textbf{FNR} \\
		\midrule
		\vulcan (This work) & 60 (3) & 59 & 60 & 2 & 40 \\ 
		\vuldl & 51 (2)& 44 & 63 & 1 & 37 \\ 
		\nb & 5 (0) & 3 & 36 & 46 & 64 \\ 
		\midrule
		\bowtok & 18 (0) & 10 & 70 & 22 & 29 \\ 
		\bowpath & 30 (0)& 61 & 20 & 0 & 80\\ 
		\vullr & 23 (0) & 17 & 35 & 1 & 65 \\
		\vulcanab & 52 (1) & 45 & 60 & 3 & 40 \\ 
		\vulcanpl & 53 (3) & 53 & 53 & 2 & 47 \\ 
		\vulcanattn & 52 (2) & 54 & 51 & 2 & 49\\ 
		\bottomrule
\end{tabular}
\caption{Vulnerability classification of different models evaluated in our work.~
All values are percentages rounded to the nearest integer.~
This is a binary classification task of classifying whether a line has a vulnerability or not.
~The results are an average of 5 independent runs each.
~P, R stand for Precision and Recall respectively.
~For readability, we show standard deviations in brackets ($\cdot$) only for F1-scores.}
\label{table}
\end{table}
%</tabl>

%<*errbars>
\begin{figure}[hbt]
	\resizebox{\linewidth}{!}{
		\includegraphics[width=\linewidth]{img/errbars.jpg}
	}
	\caption{A description for error bars of F-1 scores tabulated in Table \ref{table}}
	\label{errs}
\end{figure}
%</errbars>


%<*corr>
\begin{figure*}[htb]
	\begin{minipage}{0.7\linewidth}
		\resizebox{\linewidth}{!}{
			\includegraphics[width=\linewidth]{img/programs.png}
		}
	\end{minipage}
	\begin{minipage}{0.3\linewidth}
		\resizebox{\linewidth}{!}{
			\includegraphics[width=\linewidth]{img/dists.png}
		}
	\end{minipage}
	\caption{\textbf{How informative are line representations?} We set up three categories of synthetic \solidity programs containing 50 programs each. Categories \modd and \nomod modify unique programs in category \base in a controlled and specific manner (details in Section \ref{resultsline}). We compare the representations of specific lines of interest in programs from each of these categories as computed by a trained \vulcan. We compare the average $L^2$-distances of these representations among the three categories (right). Larger values indicate the representations are farther apart.}
	\label{pgm}
\end{figure*}
%</corr>



%<*lineembed>
\begin{figure*}[hbt]
    \resizebox{0.8\textwidth}{!}{
        \includegraphics[width=\textwidth]{img/embedding.png}
    }
    \caption{\textit{Line level embedding generator}. This corresponds to Step 4 in Figure \ref{overview}. An embedding for a line is generated by taking as inputs the embeddings corresponding to the paths of each of the tokens in that line (output of Network A) and creating one embedding using a feedforward network (Network B). The resulting embedding is then concatenated with the line embeddings of the end-points in those tokens' paths to produce the overall embedding for the line (output of Network C). See Section \ref{sec:model} for details.}
    \label{flow2}
\end{figure*}
%</lineembed>

